RAG-WM: An Efficient Black-Box Watermarking Approach for Retrieval-Augmented Generation of Large Language Models

In recent years, tremendous success has been witnessed in Retrieval-Augmented Generation (RAG), widely used to enhance Large Language Models (LLMs) in domain-specific, knowledge-intensive, and privacy-sensitive tasks. However, attackers may steal those valuable RAGs and deploy or commercialize them, making it essential to detect Intellectual Property (IP) infringement. Most existing ownership protection solutions, such as watermarks, are designed for relational databases and texts. They cannot be directly applied to RAGs because relational database watermarks require white-box access to detect IP infringement, which is unrealistic for the knowledge base in RAGs. Meanwhile, post-processing by the adversary's deployed LLMs typically destructs text watermark information. To address those problems, we propose a novel black-box "knowledge watermark" approach, named RAG-WM, to detect IP infringement of RAGs. RAG-WM uses a multi-LLM interaction framework, comprising a Watermark Generator, Shadow LLM & RAG, and Watermark Discriminator, to create watermark texts based on watermark entity-relationship tuples and inject them into the target RAG. We evaluate RAG-WM across three domain-specific and two privacy-sensitive tasks on four benchmark LLMs. Experimental results show that RAG-WM effectively detects the stolen RAGs in various deployed LLMs. Furthermore, RAG-WM is robust against paraphrasing, unrelated content removal, knowledge insertion, and knowledge expansion attacks. Lastly, RAG-WM can also evade watermark detection approaches, highlighting its promising application in detecting IP infringement of RAG systems.

==> overview.tex <==
\section{Motivation}
\label{sec:Motivation}


\begin{figure}[t]
\centering
\epsfig{figure=fig/motivation.png, width=0.5\textwidth} 
\caption{\textbf{Motivation Example}}
\label{fig:motivation}
\end{figure}






\subsection{Threat Example}
\shengzhi{Motivation examples means you tell a story: a) A model owner releases their model (complicated and accurate) on github, b) adversary identifies its value and clones it, c. To avoid legal issues, adversary fine-tunes (XXX approaches) the model and adds his own watermark, d) Adversary commercializes it (make it black box as well) and gets revenue. Then you want to use the story to emphasize the need of our approach: a) black box model from adversary, so we need to probe. But since the model is complicated and adversary has done pruning, the results of probing may not be convincing. Therefore, white box verification is needed.}

As the advance of AI techniques, neural networks are involving in various complicated tasks, e.g., autonomous driving, speech recognition, remote diagnosis, etc. Such tasks usually rely on DNN models trained on a large amount of data using intensive GPU resources.
For instance, AlexNet paper[] it’s stated that “our network takes between five and six days to train on two GTX 580 3GB GPUs”. \shengzhi{Give an example of a real world complicated model trained using XXX data and XXX GPU for XXX days.} Hence, the IP of DNN models has become a vital topic in the AI community. 

Consider an example as shown in Figure\ref{fig:motivation}, Alice makes great efforts to design a complicated and accurate neural network $DNN_{Alice}$ that performs well on the main task, and embed a backdoor[] watermark to $DNN_{Alice}$. Then he publishes $DNN_{Alice}$ to models sharing platform, such as GitHub and Google Cloud AI platform []. After that, an attacker Bob thinks that $DNN_{Alice}$ is very valuable, and then stealing it. To avoid legal issues, Bob fine-tunes, prunes the model and adds his own backdoor[] watermark, generating $DNN_{Bob}$. Next, Adversary commercializes it in black box and gets revenue.  

In view of this situation, Alice needs to claim ownership of the stolen model $DNN_{Bob}$. Alice first performs black box verification on $DNN_{Bob}$, but at this time, Bob can also have some key samples constructed by AEs or from his new constructed backdoor for fraudulent claims of ownership. Moreover since the model is complicated and adversary has done pruning, the results of probing by backdoor may not be convincing. 

%\begin{figure}[t]
%\centering
%\epsfig{figure=fig/table_attacker.png, width=0.5\textwidth} 
%\caption{\textbf{Capability of Attacker}}
%\label{fig:table_attacker}
%\end{figure}

\begin{table}
\centering
\footnotesize
\caption{Capability of Watermark}
\label{tab:Capability of Attacker}
\begin{tabular}{m{2.5cm}
<{\centering}|m{1.5cm}
<{\centering}|m{1.5cm}
<{\centering}|m{1.4cm}
<{\centering}}
\hline
\textbf{ }& \textbf{Elementary level}& \textbf{Intermediate level}& \textbf{Advanced level}\\
\hline \hline
\textbf{Fraudulent claims of ownership} & \text{\Checkmark}& \text{\Checkmark}& \text{\Checkmark}\\ \hline
\textbf{Access to White Box}& \text{-} &\text{\Checkmark}& \text{\Checkmark} \\ \hline
\textbf{Pruning and Fine-tuning}& \text{-} &\text{-}& \text{\Checkmark} \\ \hline
\textbf{Watermark Rewrite}& \text{-} &\text{-}& \text{\Checkmark} \\ \hline
\end{tabular}
\end{table}

\shengzhi{The Table needs revision. It should show how existing works and ours perform on those metrics listed in the first column.}

Moreover, we classify several levels of attackers according to the capability our attacker can have as show in Figure \ref{fig:table_attacker}.
These attackers cause great challenges to current backdoor watermarking methods. Therefore, some watermark that can play an arbitration role in ownership verification is needed, we propose $HufuNet$ which can give an arbitration result of ownership in white box. Only in this way, can Alice verify the ownership of $DNN_{Bob}$ without any controversy.


\begin{comment}
A well-trained DNN is a valuable intellectual property (IP) for its owners, officials hope to use legal measures to protect the intellectual property of model owners. And the role of the watermark is primarily to protect the IP from being infringed.

The potential security risks of the IP of DNN are watermark removing and fraudulent claims of ownership. In terms of watermark removing, previous work \textcolor{red}{[leveage] [fine-prune] [evasion]} showed that attacker $\mathbb{A}$ can increase learning rates to fine-tuning or pruning to effectively remove the black box watermark. In terms of fraudulent claims of ownership, attacker $\mathbb{A}$ can generate some AEs [X] to fraudulent claim of ownership. Both of these risks are huge challenges to black box watermark. To address the above problems, we propose a new watermark ownership framework that provides the first black box verification, and then white box ownership verification with a high robustness protection mechanism.

For the $DNN_{valid}$ of disputed ownership, we first perform a robust black box watermark verification. If the verification result is under a high degree of confidence, we will prove the ownership of $DNN_{valid}$. But in the following two cases, the black box watermarking is not enough to verify ownership, and we will utilize the more robust and trustworthy white box watermarking method. 
(1)The black box method does not prove our ownership with a high degree of confidence, but we found out it is our model through a few minor details, and then we take legal means to get the white box model of $DNN_{valid}$ for further verification. (2)Fraudulent claims of ownership. Although we can verify ownership in the black box, attackers can also generate some adversarial samples and verify them in black box. 
Similarly, we take legal means to get the white box model of $DNN_{valid}$ and performs white box verification.
\end{comment}

\begin{comment}

\subsection{Threat Model}

\shengzhi{Usually threat model is to assume the maximum capability your adversary can have. Then your approch is to deal with the worse case based on your threat model.}

The main methods of attack to eliminate the DNN watermark are pruning, fine-tuning, and watermark rewriting. Also fraudulent clams ownership attack leads to disputes over ownership. As far as these attack methods proposed, We classify several levels of attackers $\mathbb{A}$ according to the maximum capability our attacker can have as follows:

Elementary level: $\mathbb{A}$ cannot get our white box model, nor has ability of pruning, fine-tuning, watermark rewrite to our model. But he claim the ownership of our DNN rascally without any evidience.

Intermediate level:$\mathbb{A}$ does not have access to our white box model. However, they generate some AEs through queries, which in turn build trigger sets to claim ownership of the black box DNN.

Advanced level: $\mathbb{A}$ can obtain the white box model, then without pruning, fine-tuning and rewriting watermark to model. $\mathbb{A}$ didn't embed the watermark, but claimed that part of the neural network was his watermark.

Ultimate level: $\mathbb{A}$ can get access to the white box model and perform operations such as pruning and fine-tuning, further adding a similar white box secret key to claim ownership.

\end{comment}



\subsection{Design Requirements}
\shengzhi{Based on the threat model, here you can elaborate the design requirements, e.g., effectiveness, fidelity, robustness, integrity, security, etc.}

As mentioned above, we assume that attackers have a certain amount of destructive power and therefore some technical challenges need to be addressed for achieve accurate and efficient verification of watermark ownership. We conducted an in-depth analysis of the capabilities of the four levels of attackers in order to propose an excellent watermark approach.
\begin{comment}
Elementary level: Since the attacker $\mathbb{A}$ cannot get our white box model and cannot build trigger sets to verify ownership in black box, we need to design a watermark with good quality of effectiveness and integrity and security in black box verification. 

\end{comment}

Elementary level: The attacker $\mathbb{A}$ can generate some AEs to generate his trigger sample to claim ownership of our DNN, even without access to our DNN. It is a drawback to backdoor watermark to defend the attack fraudulently claim ownership. So we need to design a new watermark total different from backdoor watermark to avoid the drawback of backdoor. The new watermark shall meet the requirement as: it only can  verify the ownership of DNN which it embedded; it is difficult to fake a substitute watermark to claim ownership.

Intermediate level: Owning $\mathbb{A}$ can obtain the white box DNN and claimed that a originally part of the DNN was his watermark. In this case, we must sure our watermark with quality that watermark is undetected by attacker and it is difficult to fake a substitute watermark only by some original part of DNN and attack's local secret.


Advanced level: Due to $\mathbb{A}$ gaining the white box model, and attacking our watermark by pruning, fine-tuning, and watermark rewriting. Therefore, we need to make sure the white box watermark is of good robust to these attacks and undetected by adversary.

Moreover, a well watermark should have guaranteed a good quality that after embedding watermark, the protected DNN can not have a significant decrease in performance.

\vspace{5pt}

==> template/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

